An Empirical Study on Leveraging Images in Automated Bug Report Reproduction

Automated bug reproduction is a challenging task, with existing tools typically relying on textual steps-to-reproduce, videos, or crash logs in bug reports as input. However, images provided in bug reports have been overlooked. To address this gap, this paper presents an empirical study investigating the necessity of including images as part of the input in automated bug reproduction. We examined the characteristics and patterns of images in bug reports, focusing on (1) the distribution and types of images (e.g., UI screenshots), (2) documentation patterns associated with images (e.g., accompanying text, annotations), and (3) the functional roles they served, particularly their contribution to reproducing bugs. Furthermore, we analyzed the impact of images on the performance of existing tools, identifying the reasons behind their influence and the ways in which they can be leveraged to improve bug reproduction. Our findings reveal several key insights that demonstrate the importance of images in supporting automated bug reproduction. Specifically, we identified six distinct functional roles that images serve in bug reports, each exhibiting unique patterns and specific contributions to the bug reproduction process. This study offers new insights into tool advancement and suggests promising directions for future research.

==> pages/approach.tex <==

\section{Proof-of-Concept Approach} 

We developed a proof-of-concept tool for bug reproduction that leverages insights from our empirical study. This tool, ~\Name{}, incorporates multimodal large language models (LLMs) to automatically reproduce bug reports that include images. 
%
This tool follows a two-phase approach: the first phase classifies the functionalities of images within the bug report, and the second phase focuses on the bug reproduction process.

The overall implementation is inspired by recent works, such as AdbGPT~\cite{feng2024prompting} and ReBL~\cite{wang2024feedback}, which showcase efficient workflows and highlight the remarkable capabilities of large language models (LLMs) in automated bug reproduction. Like these approaches, our tool follows a similar workflow, where the required information is provided to the LLM to facilitate decision-making and guide the bug reproduction process effectively. The information provided to the LLM includes custom prompt instructions, GUI details, available actions and other relevant inputs needed to accurately reproduce the bug.

Our approach stands out by being multimodal, allowing the tool to accept images as input alongside text, which fill the gap that state-of-art tools does not consideer images in bug reports. Unlike other methods that rely on author discussions or experimental setups, our prompt instructions and other essential inputs are derived from and inspired by findings from an empirical study. This ensures that the information provided to the LLM is not only data-driven but also reflective of real-world scenarios, enhancing the accuracy and effectiveness of the bug reproduction process.
%



\subsection{Phase1: Classify Image Roles}
The first phase of our approach is to classify images in bug reports. RQ1 identified six distinct categories for images, each serve different purpose associated with varying patterns in the bug reports. Additionally, RQ1 revealed that  certain percentage of images are not placed in appropriate locations, making them difficult to interpret. The entire bug reports with images could lead to an overwhelming amount of information, increasing complexity and the potential for misunderstanding. To address this, categorizing images offers a more structured and efficient method. By classifying the images upfront, we can preprocess the bug reports, ensuring that each image is appropriately categorized. This helps reduce confusion, making  images in bug reports easier to interpret and leveraged for the bug reproduction.




\textbf{Prompt Design.} To enable the LLM to classify images effectively, we use the findings from RQ1 to construct the prompt. The six distinct image categories identified form the basis of our domain. Each category is accompanied by specific characteristics and patterns, helping GPT to consider not just the image itself but also its placement and context within the bug report. This prompt guides the LLM in recognizing the functional role of each image, ensuring more accurate classification.


\subsection{Phase2: Bug Reproduction}
The second phase is bug reproduction which is to explore the apps to reproduce the reported bug.
The process involves an iterative interaction with the LLM API, where at each step, we provide specific inputs, and LLM returns suggested actions.
This workflow is well adopted by existing works that use LLMs in bug reproduction or android testing.


\textbf{LLM Decision-Making.} Automated bug reproduction leveraging LLMs typically requries prompt(e.g. instructions, chain-of-thought), bug report information(e.g. S2Rs), and UI Information. Our approach introduces two key differences. We preprocess the bug report in phase 1 by classifying images in bug reports. 
%
Second, existing methods rely on textual descriptions of UI elements, using attributes like resource IDs, text labels, or content descriptions to represent the UI. Building upon their work, our tool enhances this by providing both textual information and annotated screenshots of the current UI. This approach allows for a more accurate comparison between the images in the bug report and the actual interface. By combining visual elements with text, our tool enables more precise decision-making and a deeper understanding of the bug's context, ultimately leading to more effective bug reproduction.

Figure~\ref{fig:decision} shows an example where the Step to Reproduce (S2R) is "click on the tab displaying the point," accompanied by an image indicating the target element, which is the display point. To enable LLM to accurately suggest the correct display point and corresponding action, we provide the UI information in two ways: (1) list UI elements that allows user interact (as shown in Figure 2 under "UI Information of the Current Page"). (2) An annotated screenshot of the current page,  with each UI element clearly labeled by a unique number corresponding to the clickable elements in the textual UI information. By integrating these three components—bug report infomration, textual UI information and annotated screenshots - GPT is able to precisely identify the correct target and recommend the appropriate action for reproducing the given step.
 




\begin{figure}[h]
    \centering
    \includegraphics[width=0.95\linewidth]{figures/ui.png}
    \caption{Essential Information for LLM-Based Decisions}
    \label{fig:decision}
\end{figure}







\subsection{Implementation}\commentdbw{copy from crashtranslator}
We implement our approach in Python and extend functionalities from the following libraries: Appium [1] to interact with Android apps and obtain the view hierarchy of the current page; NLTK [43] to stem word, which is used in the widget hitting scorer (Section 3.3); Ella [16] to check whether crash-involved APIs are triggered, which is used in the exploration optimization scorer (Section 3.4); OpenCV [45] to mark widgets that need to be interacted with on screenshots, which is used in generating reproducing steps (Section 3.5). We run CrashTranslator and perform experiments on a physical x86 Ubuntu 20.04 machine with Android emulators (Android 4.4-7.0).
For the LLM leveraged in the page reaching scorer (Section 3.2), we adopt the pre-trained GPT-3 [4] model from OpenAI3. We choose the Curie model as the base model and fine-tune the model through official APIs as described in Section 3.2. Developers only need to set up their OpenAI account, complete the fine-tuning process according to the instructions provided on our website2, and subsequently utilize our tool to automatically. On average, reproducing one crash requires sending approximately 42.6 prompts (4939.7 tokens), with an estimated cost of around 0.01 USD.


==> pages/evaluation.tex <==





\section{Evaluation and Results of \Name{}}
We conducted a thorough evaluation of \Name{}'s performance. Given that our approach involves two primary phases, we evaluate each phase separately: 
Classify Image Roles and Guided Replay.

\begin{itemize}[leftmargin=0.35cm]
    \item RQ1: How accurate is our approach in classifying images in bug reports?
    \item RQ2: How accurate is our approach at reproducing image bug reports?
\end{itemize}


\subsection{RQ1: Accuracy of Image Role Classification}

\subsubsection{Metric} Accuracy is the metric used to evaluate \Name{}'s performance in classifying image roles. t is defined as the ratio of correct classifications to the total number of images. The correctness of these classifications is validated by comparing the results against the ground truth, which is manually established by the authors following the methodologies and findings of the empirical study (Section~\ref{}).

\subsubsection{Baselines}
We included two ablated versions as baselines in our analysis: 
\textbf{\(\Name{}_{\text{BasicPrompt}}\)} uses basic prompt containing only essential instructions to guide the LLM in automating the classification process. By including core task specifications and relevant image roles, it ensures responses stay within the required domain for effective workflow execution.
%
\textbf{\(\Name{}_{\text{OrigImg}}\)} uses the original images from bug reports without embedding the image IDs at the top as titles.
In contrast, the full version of \textbf{\Name{}} incorporates both chain-of-thought reasoning and embedded images. We use two baselines to evaluate the impact of chain-of-thought reasoning and image embedding on improving the effectiveness of image classification in bug reports.

\begin{table}[h]
\centering
\begin{threeparttable}
\caption{Evaluation of Classifying Images}
\label{result1}
\begin{tabular}{|c|c|c|c|}
\hline
 \rowcolor{gray!30} Tool & Single-Image Reports & Multi-image Reports & Overall \\
\hline
\Name{}_{\text{BasicPrompt}} & 90.56\% & 57.39\% & 77.63\% \\
\hline
\Name{}_{\text{OrigImg}} & 93.33\% & 53.91\% & 77.97\% \\
\hline
\textbf{\Name{}} & 96.11\% & 60.00\% &  \textbf{82.03\%} \\
\hline
\end{tabular}
\begin{tablenotes}
\footnotesize
\item[1] Single-Image Reports refer to reports with only one image; Multi-Image Reports refer to reports that include more than one image.
\end{tablenotes}
\end{threeparttable}
\end{table}



\subsubsection{Result.}
The evaluation results (Table~\ref{result1}) demonstrate that our proof-of-concept tool achieves 82.03\% accuracy outperforms the two ablated versions. This result highlights the necessity of integrating detailed reasoning and image annotation to improve classification performance.

The absence of systematic classification instructions and the lack of chain-of-thought reasoning hindered \textbf{\(\Name{}_{\text{BasicPrompt}}\)}'s ability to accurately classify images.
%
Additionally, the lack of annotated images caused \textbf{\(\Name{}_{\text{OrigImg}}\)} to struggle when classifying images in bug reports that included multiple images, as it faced difficulty maintaining associations between the text and the images. However, the use of original images without embedding did not negatively impact single-image reports, as there were no issues of associating an image with the text when only one image was involved. This explains why \textbf{\(\Name{}_{\text{OrigImg}}\)} achieved 93.33\% accuracy in single-image reports but performed the worst among the three versions for multi-image reports, achieving only 53.91\%, even lower than \textbf{\(\Name{}_{\text{BasicPrompt}}\)}.


Although our proof-of-concept tool achieves an accuracy of 82.03\% in classifying images in bug reports, there are still some challenges.  several challenges remain. Specifically, the accuracy drops to 60\% when handling reports with multiple images. The primary reasons for this are: (1) Poor Documentation in Multi-Image Reports: Users often include multiple images in bug reports without providing explanations for each, leading to ambiguity and inconsistency. (2) Limited Ability to Capture Minor Details: The tool currently lacks the sensitivity to identify subtle information in images, which is often critical for accurate classification.


\begin{tcolorbox}[colback=gray!15, colframe=black, ]
{\bf Insights of RQ1:}  {
%
1. Bug Report Templates: Advise users to avoid multiple screenshots without context; add brief text or annotated highlights.
%
2. Pretrained models and prompt engineering alone may miss UI details. Enhanced visual tools or specialized training may be needed to improve accuracy.

}
\end{tcolorbox}




\subsection{RQ2: Effectiveness of Replaying S2R includes Images}

\subsubsection{Metric.} \Name{}'s performance in translating S2R image is assessed using accuracy as the primary metric. Accuracy is determined by dividing the number of correctly interpreted S2Rs by the total number of S2Rs evaluated. An S2R is deemed correctly interpreted when it fully and accurately translated into executable action with related target, input, and direction, if applicable. To establish the ground truth, the authors manually reproduce each bug report and meticulously document the correct reproduction sequence.

\subsubsection{Baselines}
\commentty{Justify the rationales of
adopting different baselines.}
Three ablated versions were used as baselines in the analysis to assess \Name{}' overall performance and the contribution of  different components:  \(\Name{}_{\text{BasicPrompt}}\)，  \(\Name{}_{\text{NoAnnoted}}\) and 
\(\Name{}_{\text{OnePhase}}\).
%
\textbf{\(\Name{}_{\text{BasicPrompt}}\)} utilizes zero-shot learning as opposed to few-shot learning.
%
\textbf{\(\Name{}_{\text{NoAnnoted}}\)}  excludes an annotated UI screen, providing only a textual description of the current UI information and a plain screenshot.
%
\(\Name{}_{\text{OnePhase}}\) merges phase 1 and phase 2 to evaluate the necessity of separating image role classification and replay.
%
The full version of\textbf{ \Name{}} incorporates few-shot learning, the chain of thought approach, annotated UI screenshots, and utilizes the processed bug report from phase 1 as input.

\subsubsection{Result.} 
The evaluation results

\subsection{Discussion}
The simple implementation shows its promise in reproducing image bug report, which complements existing tools. 
We leave such optimizations as future work.

==> pages/xxx.tex <==
\subsubsection{Documentation of Images} 

%\commentdbw{placement? explanation? documentation?}} 

Unlike GIFs or videos, which capture the entire process of triggering a bug (including every UI page, actions, and transitions between pages), images are limited to presenting a snapshot of a specific UI state. Just as roles need to be identified in textual descriptions (e.g., determining whether a sentence is a S2R), fully leveraging image information for bug reproduction requires labeling the functional roles of images 
(i.e., the six categories described in Section 3.1). This helps facilitate the bug reproduction process. For instance, existing tools use S2R sentences as input to guide reproduction; similarly, images need analogous roles to be effectively utilized. 

We analyze how images are documented in bug reports to ascertain their functional roles. A well-documented image includes sufficient context to identify its function, such as the caption of the section where it's placed or the accompanying text, which clearly communicates its role within the report. Identifying an image’s appropriate role can often be achieved using simple regular expressions. For example, an OB (Observed Behavior) image appearing under a section titled "Observed Behavior" or "Actual Behavior" is considered well-aligned because its purpose aligns with that of the section, both aiming to illustrate the observed issue.
%
In contrast, if an image is placed out of its appropriate section, it requires additional effort to determine the role of the image,
such as using classification techniques. 

%In such cases, 
%readers must interpret the whole bug report to accurately identify whether the image is related to OB, EB, or S2Rs. If it is related to S2Rs, further interpretation is needed to determine which specific S2R it relates to.

Table ~\ref{tab:location} presents the well-documented image of each role. OB Image has the lowest proportion, with xx\% of OB images being incorrectly placed.

%Additionally, among the total xx wrong placement images, xx\% were OB iamge, and xx\% are the single image in the bug report.This is  likely occurs because the template provides a designated area for images, while the latter may be due to the perception that placing images at the end of the document makes it easier to organize.

%We find that xx\% (xxx/xxx) of wrongly placed images are located in a section called 'Screenshots.' Of these, xx\%(xxx/xxx) contain only one image, while xx\% have more than one image. When there is only one image, xx\% are OB images. However, when there are multiple images, it becomes not only challenging to identify their roles but also difficult to understand their relationships.





%Considering that user writing habits and preferences can lead to inconsistencies that make bug reports less readable and harder to understand, we also examine whether the images are positioned correctly. Correct positioning is defined, for example, as an OB Image appearing in the OB section of the report. Images placed outside their designated sections are deemed incorrectly positioned.


\begin{tcolorbox}[colback=gray!5, colframe=black, ]
{\bf Finding 4:}  {
%
XX\% of poorly documented images are placed separately at the end  or in the “screenshot” section of the bug report without any description, with the majority (xx\%) of them are OB Image. Therefore, approaches on identifying specific roles of images are needed
}
\end{tcolorbox}


%
\begin{table}[h]
    \centering
    \scriptsize
    \hspace*{\fill}
    \begin{minipage}{0.45\linewidth}
        \centering
        \begin{threeparttable}
        \caption{Distribution of Bug Reports Containing Images Across Different Functionalities} 
        \label{tab:roles}
        \begin{tabular}{l|l|*{6}{>{\centering\arraybackslash}p{0.325cm}}}
            \toprule
              & \# BR & S2R\_s & S2R\_c & S2R\_r & OB & EB & Others \\ \hline
            \textbf{Our Dataset}  & -    &  0.4\%   & 9.8\% & 2.9\%       & 94.7\%    & 18.0\% & 6.5\%     \\
            AndroR2   & 36 & 0\%  & 11.1\%      & 8.3\%    & 100\% & 5.6\%  & 5.6\%      \\
            RegDroid  & 162 & 0.6\%  & 4.3\%    & 9.3\%    & 87\%    & 11.1\%  & 8.6\%     \\
            \bottomrule
        \end{tabular}
        
        \begin{tablenotes}
            \footnotesize
            \item[1] \tiny S2R\_s = S2R\_standalone, S2R\_c = S2R\_context, S2R\_r = S2R\_result
        \end{tablenotes}
        \end{threeparttable}
    \end{minipage}%
    \hfill
    \begin{minipage}{0.45\linewidth}
        \centering
        \vspace{-10pt}
        % \begin{threeparttable}
        \caption{Distribution of Well-Documented Images Across  Functionalities}
        \label{tab:location}
        \begin{tabular}{l|l|*{4}{>{\centering\arraybackslash}p{0.3cm}}}
            \toprule
              & \# Img & S2R  & OB & EB & Others\\ \hline
            \textbf{OurDataset}      &  & -  & -          & -      \\
            AndroR2  & & -  & -        & -    & -    \\
            RegDroid & & -  & -       & -    & -   \\
            \bottomrule
        \end{tabular}
         %\begin{tablenotes}
        %    \item[1] \tiny S2R = the sum of all three kinds of S2R image
       % \end{tablenotes}
       % \end{threeparttable}
    \end{minipage}
    \hspace*{\fill}
\end{table}


\subsubsection{Generalizability of RQ2}
\label{represent}
\commentty{need more explanation.}
Generalizability is crucial for RQ₂, which focuses on analyzing the utilization of images in bug reports within a randomly sampled dataset. To ensure that our findings are not limited to the specific characteristics of this initial sample, we validated our results by applying the same analysis to two independent third-party datasets 
 AndroR2~\cite{wendland2021andror2, johnson2022empirical} and RegDroid~\cite{xiong2023empirical}.  
 
 %The two datasets were not constructed by the authors of this paper, and the presence of images in bug reports was not one of the criteria in their construction, nor were images in bug reports studied in subsequent analyses. \commentty{what is the purpose of the above sentence?}
%In contrast, RQ2 does not require generalizability because its goal is to evaluate the impact of images through controlled experiments using existing bug reproduction tools, with and without image information. This approach is designed to measure the effectiveness and efficiency under specific conditions, providing insights into how images influence tool performance rather than establishing a broad understanding of common practices or patterns.
AndroR2 contains 30\% (39/130) of bug reports with images,though three of these reports either no longer have access to the images or the images are externally hosted. For RegDroid, 41.85\% (167/399) of bug reports include images, but five of these reports lack access to the images. We focused on bug reports with accessible images, which includes 36 from AndroR2 and 162 from RegDroid. We applied the same methodologies (as described in Section~\ref{method}) used in RQ1 to classify the images in the bug reports and assess their placements. The results were then compared to our own dataset to determine if the findings from these third-party datasets align with ours. This analysis helps assess the representativeness of our findings.

%
Table~\ref{tab:roles} and Table~\ref{tab:location} present the results of classifying image roles and assessing image placement for our dataset and the two third-party datasets. The findings reveal a consistent trend: most bug reports feature OB images, with S2R images being the second most prevalent. The similar distribution of image roles across all three datasets indicates that our study's findings are generalizable beyond the randomly sampled dataset. By classifying and evaluating images in AndroR2 and RegDroid, we demonstrate that the identified patterns are consistent across different data sources and contexts. This cross-validation confirms the robustness of our findings regarding the utilization of images in bug reports, thereby enhancing the validity and reliability of our conclusions.





\ignore{
\subsubsection{Methodology}
Two authors independently classified the role of images and then cross-validated their results through comparison and discussion. When consensus could not be reached, an additional author was consulted to ensure agreement on the final categorization. The followed the follwing steps to classif

\begin{itemize}[leftmargin=0.5cm]
\item  The placement of images of bug reports often reveals their roles, particularly in reports that adhere to well-defined templates. Structured bug reports clearly organize information into titled sections, making categorization straightforward. For example, For example, an image located within the OB section can be distinctly classified as an OB image. 

\item Contextual analysis is essential for classifying images in unstructured bug reports and S2R images. This is because unstructured bug reports lack titled sections, and S2R images fall into three subroles, as introduced in section ~\ref{}. By examining the surrounding text and overall content, the role and relevance of each image can be accurately determined, ensuring proper classification.

\end{itemize}
}
